Circulation Statistics in Homogeneous and Isotropic Turbulence

This is the final version of a Thesis presented to the PostGrad Program in Physics of the Physics Institute of the Federal University of Rio de Janeiro (UFRJ), as a necessary requirement for the title of Ph.D. in Science (Physics). The development of the Vortex Gas Model (VGM) introduces a novel statistical framework for describing the characteristics of velocity circulation. In this model, the underlying foundations rely on the statistical attributes of two fundamental constituents. The first is a GMC field that governs intermittent behavior and the second constituent is a Gaussian Free field responsible for the partial polarization of the vortices in the gas. The model is revisited in a more sophisticated language, where volume exclusion among vortices is addressed. These additions were subsequently validated through numerical simulations of turbulent Navier-Stokes equations. This revised approach harmonizes with the multifractal characteristics exhibited by circulation statistics, offering a compelling elucidation for the phenomenon of linearization of the statistical circulation moments, observed in recent numerical simulation. In the end, a field theoretical approach, known as Martin-Siggia-Rose-Janssen-de Dominicis (MSRJD) functional method is carried out in the context of circulation probability density function. This approach delves into the realm of extreme circulation events, often referred to as Instantons, through two distinct methodologies: The First investigates the linear solutions and, by a renormalization group argument a time-rescaling symmetry is discussed. Secondly, a numerical strategy is implemented to tackle the nonlinear instanton equations in the axisymmetric approximation. This approach addresses the typical topology exhibited by the velocity field associated with extreme circulation events.

==> aaaa.tex <==
$_{}$

Almost 200 years before Isaac Newton's formulation of classical mechanics, Leonardo da Vinci was already fascinated by the dynamics of fluid motion. Based on detailed visual observations and graphic reproductions, da Vinci developed an extraordinary physical intuition about the movement of fluid, as quoted in his notebooks \cite{da2008notebooks,mossa2021recent},
\begin{figure}[H]
\center
\includegraphics[width=\textwidth]{img/1.1.png}
\caption[Da Vinci's studies on fluid motion.]{Da Vinci's drawing on the fluid motion (The Royal Collection, RL 12659v), available online at \url{https://www.rct.uk/collection/912659/recto-studies-of-flowing-water-with-notes-verso-studies-of-flowing-water}.}
\label{fig1.1}
\end{figure}

``\textit{Observe the motion of the surface of the water, how it
resembles that of hair, which has two movements—one
depends on the weight of the hair, the other on the direction
of the curls; thus the water forms whirling eddies, one part
following the impetus of the chief current, and the other
following the incidental motion and return flow.}'' 

Figure~\reffig{fig1.1} is one of the several fascinating originals of da Vinci's drawings of chaotic fluid motion. It predicts the prevalence of vortical swirling structures, as well as the view of motion as a superposition of a main flow and random fluctuations. These ideas form the building rock of all modern interpretations of turbulent fluid flow phenomena. The very creation of the term ``turbulence'' can be traced back to da Vinci (``\textit{turbolenza}'' derived from ``\textit{turbare}'', meaning ``perturb'' or ``became agitated'' in Italian), although its use in scientific literature is attributed to William Thomson a.k.a. Lord Kelvin \cite{lambd1932hydro,thomson1887xlv}.

After Newton's formulation of the laws of mechanics in 1687 \cite{newton1687}, the conceptualization of several ideas changed the way we understand motion. Concepts such as space, velocity, momentum, mass, energy, and inertial frames emerged and successfully described the motion of particles and rigid bodies. Thus, the application of fluid flow was a very natural step with several technological applications at the time such as naval advancements, canal and dam constructions, and ancient challenges like the desire to fly or at least comprehend the mechanisms of flight. The theoretical challenge was also intriguing: if Newtonian mechanics elegantly and precisely described the motion of rigid bodies, how could it be applied to fluid flow? How could it account for the diverse range of behaviors and phenomena that arise under different conditions of fluid flow? Is there possible to comprise in a single equation the transition from the typical smoothly flowing stream (laminar flow) to the apparent disordered motion of a waterfall (turbulent flow)? 

In the words of the Nobel laureate Richard Feynman, written in his famous Lectures on Physics series \cite{feynman1964feynman}:

``\textit{Often, people in some unjustified fear of physics say you can't write an equation for life. Well, perhaps we can. As a matter of fact, we very possibly already have the equation to a sufficient approximation when we write the equation of quantum mechanics: $\hat{H}\psi=i\hbar\dot{\psi}$}.''

In the context of fluid dynamics and turbulence, the ``equation for life'' referred to by Feynman is believed to be the \ac{iNSE}. It is one of the few problems in history which resisted the analysis of several noble names in science like I. Newton (1663---1727), D. Bernoulli (1700---1782), L. Euler (1707---1783), J.-L. Lagrange (1736---1813), C.-L. Navier (1785---1836), Sir G. Stokes (1819---1903), Lord Kelvin (1824---1907) and many others.

The \ac{iNSE} and its energy-conservative version (Euler equations) have captured the attention of mathematicians due to their simple form. Within this context, even the fundamental question about the existence and smoothness of solutions for these equations continues to avoid a mathematically formal solution. This enduring challenge motivated the Clay Mathematics Institute to attach a substantial US\$ 1 million prize to its resolution as a Millenium Prize Problem. The exact statement of the Millenium Problem can be found in a short paper by Fefferman \cite{fefferman2000existence}. In short, the question addressed is: Given smooth initial conditions, do the evolution of the solutions maintain their regular and analytical characteristics for a finite duration, or if they succumb to singularities?

As the \ac{iNSE} plays an important role in the dynamics of fluids, let's do a modern still elementary derivation of these equations, fixing notations and definitions.

\section{Incompressible Navier-Stokes Equations}\label{sec1.1}

$_{}$

Every matter in the universe, in the classical physics sense, is constituted by atoms and molecules with well-defined properties like mass, charge, etc. However, the development of fluid dynamics happened much before the atomistic theory of matter ($20^{th}$ century). Instead, fluids (liquid and gases) are treated as continuum media since any small volume element in the fluid is always supposed so large that it still contains a very great number of molecules \cite{landau2013fluid}. For example, atmospheric air at ambient temperature and pressure has, in a small cube of side $10^{-3}$ cm, an order of $3\times10^8$ molecules. This number is larger for liquids such as water since its density is about $10^3$ times air's density. In this sense, the fluid is macroscopically described by quantities that vary with continuous position $\vc x$ and time $t$ indexes, such as velocity $\vc v(\vc x,t)$ and pressure $p(\vc x,t)$. The latter is called the Eulerian point of view in fluid dynamics, in which the coordinates refer to a fixed reference frame. There is also the Lagrangian frame, in which individual parcels of fluid are tracked, and the position index refers to small fluid elements.

The fluid dynamics equation derives directly from two basic concepts in Newtonian mechanics: mass conservation and the momentum equation (second Newton's law). The former can be simply stated as follows\footnote{Repeated indices are summed following Einstein's notation unless explicitly stated. Moreover, no distinction will be made among covariant $x_i$ and contravariant $x^i$ indexes, since we are working with Euclidian spaces and cartesian coordinates such that the metric $g_{ij}=g^{ij}=\delta_{ij}$.},
\be\label{1.1}
\partial_t\rho+\partial_i\big(\rho v_i\big)=0\ ,\
\ee
where $\rho=\rho(\vc x,t)$ is the local fluid density and $\partial_i \equiv \partial/\partial x_i$ (similarly for temporal derivatives). The momentum equation reads,
\be\label{1.2}
\frac{d}{dt}\big(\rho v_i\big)=\partial_i \sigma_{ij}[v]\ ,\
\ee
where $\sigma_{ij}$ is the Cauchy stress tensor which describes the
interaction among neighboring fluid elements with each other. In fact, the nature of the stress tensor relies upon the molecular interactions that compose the fluid. Different fluids can be classified regarding the dependency of the stress tensor on the velocity field. There exist very odd behavior fluids like cornstarch in water, silicone oils, synovial fluids, etc. The latter belongs to a class called non-Newtonian fluids such that the response of this kind of fluid to stresses is nonlinear. Newtonian fluids like water, air, liquid honey, blood plasma, and many others are characterized by linear responses when stressed, meaning for this kind of fluids the most general stress tensor assumes the form \cite{landau2013fluid},
\be\label{1.3}
\sigma_{ij}[v]=\mu\lr{\partial_i v_j+\partial_jv_i-\frac{2}{3}\delta_{ij}\partial_kv_k}+(\lambda \partial_kv_k-p)\delta_{ij}\ ,\
\ee
where $p=p(\vc x,t)$ is the pressure field and $\mu$ and $\lambda$ are the coefficients of viscosity defined in such a way that both are positive. The $\lambda$ coefficient is sometimes referred to as the second viscosity. At this point is important to assume we are dealing with barotropic fluids. A barotropic fluid is a fluid whose density is a function of pressure only $\rho=\rho(P)$. For most liquids, this assumption can be applied if the typical velocity of the fluid is not comparable to the speed of sound. Eq.~\eqref{1.1} when combined with the barotropic assumption, leads us to the condition of divergence-free velocity field $\partial_iv_i=0$. In the latter case, Eq.~\eqref{1.3} is independent of the second viscosity $\lambda$ in such a way that,
\be\label{1.4}
\partial_tv_i+v_j\partial_j v_i-\nu\partial^2v_i+\partial_iP=0\ ,\
\ee
\be\label{1.5}
\partial_iv_i=0\ ,\
\ee
where $\nu=\mu/\rho$ is the kinematic viscosity, $P(\vc x,t)=p(\vc x,t)/\rho$ is the reduced pressure (usually referred to as pressure only) and we have also used the identity for the total time derivative $\dot f(\vc x,t)=\partial_tf+v_j\partial_jf$. External forcing can be applied by adding a divergenceless function $f_i(\vc x,t)$ on the \ac{RHS} of Eq.~\eqref{1.4}. The above equations plus appropriate initial and boundary conditions are the so-called \ac{iNSE}. Note that this set of equations models a very ideal case of the huge variety of fluid motion since we assumed the barotropic approximation for simple Newtonian fluids. However, even this very simple set of equations with a unique parameter $\nu$ is the subject of mathematical ill-posedness leading to the Millenium Prize problem.

Examples of kinematic viscosities at $20^oC$ in S.I units are $1\times10^{-6},1.5\times10^{-5},2.2\times10^{-6},6.8\times10^{-4},1.2\times10^{-7}$ for water, air, alcohol, glycerine, and mercury, respectively. At first glance, Eq.~\eqref{1.4} may not seem like a closed system since it involves two different fields. However, even though the pressure is traditionally represented by the function $P(\vc x, t)$, it is not independent of the velocity field. Indeed, taking the divergence of Eq.~\eqref{1.4} and using Eq.~\eqref{1.5}, we find
\be\label{1.6}
\partial^2 P=-\partial_i \partial_j (v_i v_j)\Longrightarrow P=-\partial^{-2}\Big[\partial_i\partial_j(v_iv_j)\Big]\ ,\
\ee
where we introduced the inverse of the Laplacian operator meant to satisfy the following identity $\partial^{2}(\partial^{-2}f)=f$. This shows that pressure is given in terms of velocity through a Poisson equation, analogous to the electric potential of a distribution of charges. The solution in an infinite domain can be obtained through this electromagnetic analogy, with the known solution of Gauss's law for electric potential,
\be\label{1.7}
P(\vc x,t) =\int d^3y \frac{1}{4\pi|\vc x -\vc y|}\frac{\partial}{\partial y_j}\frac{\partial}{\partial y_j}\Big(v_i(\vc y,t)v_j(\vc y,t)\Big)\ ,\
\ee
demonstrating that we indeed have a closed system describing the evolution of the velocity field. At this point, it is interesting to note that the solution Eq.~\eqref{1.4} is non-local in space, a consequence of the classical nature of the compressibility constraint: a local change in the velocity field generates immediate effects throughout the whole space domain, instantaneously.

A different way of writing the \ac{iNSE} is by inserting Eq.~\eqref{1.6} into Eq.~\eqref{1.4} to get
\be\label{1.8}
\partial_tv_i+\mathcal{P}_{ik}\big(v_j\partial_j v_k\big)-\nu\partial^2v_i=0\ ,\
\ee
where $\mathcal{P}_{ik}=\delta_{ik}-\partial^{-2}\partial_i\partial_k$ is the projector operator into solenoidal modes. This operator extracts only the incompressible part of the fields since any $C^1$ three dimensional vector field can be decomposed into ``scalar'' and ``vector'' potentials i.e. as the Helmholtz decomposition: $f_i=\partial_i\phi+\epsilon_{ijk}\partial_jA_k$, where $\epsilon_{ijk}$ is the full antisymmetric Livi-Civita symbol. It is then clear that $\mathcal{P}_{ik}(f_k)=\epsilon_{ijk\partial_jA_k}$ completely removes the compressible part of the vector $f_i$.

Eq.~\eqref{1.8} has the advantage of depending only on the velocity field, in opposition to the system of Eqs.~\eqref{1.4} and \eqref{1.5}. The cost of it is the explicit nonlinear and nonlocal formulation of \ac{iNSE} since the explicit formulation of the projection operator involves inverse Laplacian, meaning that Eq.~\eqref{1.8} is an integral-differential equation. A rather different way of eliminating the Pressure field from the dynamic equation is to take the curl of Eq.~\eqref{1.4}, in vector notation,
\be\label{1.9}
\partial_t\vc \omega+\vc \nabla\times\big(\vc v \times \vc \omega\big)-\nu\partial^2\omega_i=0\ ,\
\ee
\be\label{1.10}
\vc \omega=\nabla\times\vc v \ ,\
\ee
where the vector identity $v_j\partial_jv_i=\partial_i(v_jv_j/2)-\epsilon_{ijk}v_j\omega_k$ was used in the above derivation. The quantity $\vc\omega$ is the so-called vorticity, a central concept in turbulence that measures the rotating ratio of a fluid element. Note that, the substitution of Eq.~\eqref{1.10} in Eq.~\eqref{1.9} to have a closed $\omega$ equation, also implies in the computation an inverse Laplacian as $v_i=\partial^{-2}(\epsilon_{ijk}\partial_j\omega_k)$ for $\partial_iv_i=0$. However, the vorticity equations are mostly used for numerical simulation of fluid dynamics equations.

\section{Transition to Turbulence and the Reynolds Number}\label{sec1.2}

$_{}$

In a classic work from 1851,  Sir G. Stokes proposed the calculation of the frictional force on a pendulum oscillating in a fluid, leading to the famous formula for drag on a sphere at low speeds \cite{stokes1851effect}. The fundamental assumption in the calculation is that for slow pendulum motion, the advection term $v_j \partial_j v_i$ is negligible compared to the dissipative term $\nu\partial^2 v_i$, allowing it to be discarded. This approximation is nowadays known as Stokes flow. Stokes' work is considered the precursor to one of the most important concepts in fluid dynamics, the Reynolds number. More precisely it associates the advection term with turbulence production and discusses the role of scales in a fluid dynamics problem.

However, this new paradigm in fluid mechanics was primarily established through the significant experimental progress of the $19^{th}$ century, especially the work of the British physicist Osborne Reynolds (1842-1912) in 1883 \cite{reynolds1883xxix}. Studying various flows in pipes, he discovered the phenomenon of transition to turbulence and demonstrated that, for a given geometry, this transition is controlled by a single dimensionless parameter, now named the Reynolds number ($Re$). 

Figure~\reffig{1.2} shows the original sketches of the experiments published by Reynolds. The experimental setup is the following: a constant flow rate is pumped in a long and thin pipe and, at the same rate but in smaller volume a jet is carried by the flow. By controlling the flow rate, the geometry of the pipe, and the liquid which is flowing, Reynolds found that the relevant dimensionless parameter that controls the different flow regimes was $Re = U_0 d/\nu$, where $U_0$ is the injection velocity, $d$ is the pipe diameter, and $\nu$ as the viscosity of the fluid. The emergence of vertical vortical structures was depicted by observing the flow through light flashes generated by electric sparks. These structures appears abruptly by varying $U_0$ and only above a critical value, beyond which the transition to turbulence occurred. He also noticed that the associated critical value of $Re$ was highly sensitive to perturbations present at the pipe entrance or in the fluid injection mechanism, demonstrating the crucial role of instabilities in turbulence creation.
\begin{figure}[t]
\center
\includegraphics[width=\textwidth]{img/1.2.png}
\caption[Reynolds' sketches on his experiments and flow past a cylinder.]{Left panel shows original sketches of Reynolds' experiments (edited from \cite{reynolds1883xxix}). The right panel shows the visualization of a fluid flow passing a cylinder at different Reynolds numbers (edited from \cite{van1982album}).}
\label{fig1.2}
\end{figure}

In a more general sense, we can think of a fluid with viscosity $\nu$ where energy is pumped at a typical scale $\ell$ controlled by external force or perturbation mechanisms. This force generates velocity differences of a typical magnitude $v_0$ between the point separated by the scale $\ell$. These thus become the scales of the problem, and according to Reynolds' proposition, flow behavior should be governed by the dimensionless parameter
\be\label{1.11}
Re = \frac{v_0\ell}{\nu}\ .\ 
\ee
The right panel of Fig.~\reffig{fig1.2} shows different regimes of the flow passing a cylinder. The Reynolds number in this geometry is calculated based on the diameter of the cylinder. Exactly as in Reynolds' experiments, the velocity field near the cylinder starts smooth for very low flow rates (a), and, as it increases, vortices start to appear in the back of the cylinder (b). As the flow rate increases these vortices detach from the cylinder to form a vortex sheet --- also known as von Kármán's sheet --- with regular spacing (c). At (d) chaotic mixing starts to play a crucial role and, in (e) the flow past the cylinder is completely chaotic and mixing i.e. turbulent.

To support this scaling behavior directly from \ac{iNSE}, we perform a change of variables at Eq.~\eqref{1.4} to dimensionless quantities: $\vc x\ ' = \vc x/\ell$ and $t' = t/\tau$, defining a typical time scale $\tau \equiv\ell/v_0$. In this case, derivatives transform as $\partial_i=\ell^{-1}\partial'_i$ and $\partial_t=\tau^{-1}\partial'_t$, while the transformation of physical quantities can be obtained through dimensional analysis. The dimensions of the fields, after setting $\rho = 1$, are represented by
\be\label{1.12}
v_i(\vc x,t) = \frac{\ell^2}{\tau^2}\bar{v}_i(\vc x\ ',t')\ ,\ 
\ee
\be\label{1.13}
P(\vc x,t) = \frac{\ell^2}{\tau^2}\bar{P}(\vc x\ ',t')\ ,\ 
\ee
and,
\be\label{1.14}
f_i(\vc x,t) = \frac{\ell}{\tau^2}\bar{f}_i(\vc x\ ',t')\ ,\ 
\ee
where the bar denotes dimensionless functions, which, however, have the same functional form as their dimensional counterparts. Substituting Eqs.~\eqref{1.12}---\eqref{1.14} into Eq.~\eqref{1.4} and renaming the variables $(\vc x\ ', t')$ back to $(\vc x, t)$, we obtain the dimensionless equations:
\be\label{1.15}
\partial_t\bar{v}_i+\bar{v}_j\partial_j \bar{v}_i-\frac{1}{Re}\partial^2\bar{v}_i+\partial_i\bar{P}=\bar{f}_i\ .\
\ee
This equation demonstrates that the Reynolds number is indeed the sole parameter that distinguishes the possible flow outcomes from the solution. It also connects the observations of Stokes and Reynolds: when $Re \ll 1$, the dissipative term dominates over the effects of the advective term, and the solution tends to be smoother, characterizing the laminar regime. When $Re \gg 1$, the opposite is true, and the advective term prevails, causing the injected energy to perturb the entire flow due to its action, defining the turbulent regime.

The question of how to define turbulence is quite nonuniversal (depending on the geometry) and reveals that the challenges in its study can be as fundamental as defining the subject itself. Now on, we will refer to turbulence as the chaotic movement of fluids characterized by large Reynolds numbers. In pipe flows, such as Reynolds' experiment, the laminar-turbulent transition is typically observed around $Re \sim 2500$ the perturbation generated by different mechanisms fills the whole pipe \cite{eckhardt2007turbulence}. Although laminar flow is able to be sustained up to $Re \sim 13000$ with meticulous control of external perturbations and fluid injection \cite{reynolds1883xxix}. In everyday situations, $Re$ can often reach values as high as $10^9$, as seen in the airflow around a car on a road or atmospheric flows, underscoring the importance of turbulence research. 

The modern understanding of the problem of turbulence only came with the experiments and theories developed in the $20^{th}$ century, as already mentioned. Besides Reynolds, other important scientists in the development of the theory of turbulence range from L. Prandtl (1875-1953), L. Richardson (1881-1953), T. von Kármán (1881-1963), and G. I. Taylor (1886-1975), who made the first discoveries on the statistical characterization of the laminar-turbulent transition, the formation of vortical structures, energy cascade, and others. Their contributions served as inspirations to the ones who came next such as J. von Neumann (1903---1957), A. Kolmogorov (1903---1987), L. Onsager (1903---1976), L. Landau (1908---1968), R.P. Feynman (1918---1988), U. Frisch (1940---), A.M. Polyakov (1945---), A.A. Migdal (1945---), and even G. Parisi (1948---) the 2021 Nobel laureate, among others. 

In particular, A. Kolmogorov built the first quantitative theory to describe these phenomena in 1941, which is nowadays widely referred to \ac{K41}. We will then attempt to establish a more precise definition related to the statistical restoration of the symmetries of the \ac{iNSE}. However, we will see that this definition cannot encompass all the richness of experimentally observed phenomena and will be associated with a specific type: fully developed homogeneous and isotropic turbulence. The rigorous and definitive definition of turbulence remains an open question, though identifying it proves to be a considerably simpler task.

\section{Symmetries and Conservation Laws of iNSE}\label{sec1.3}

$_{}$

S

\section{Outline of the Thesis}\label{sec1.4}

$_{}$

